Navigating Ensemble Configurations for Algorithmic Fairness

Bias mitigators can improve algorithmic fairness in machine learning models, but their effect on fairness is often not stable across data splits. A popular approach to train more stable models is ensemble learning, but unfortunately, it is unclear how to combine ensembles with mitigators to best navigate trade-offs between fairness and predictive performance. To that end, we built an open-source library enabling the modular composition of 8 mitigators, 4 ensembles, and their corresponding hyperparameters, and we empirically explored the space of configurations on 13 datasets. We distilled our insights from this exploration in the form of a guidance diagram for practitioners that we demonstrate is robust and reproducible.

==> fig_tree_large.tex <==
\begin{figure*}[!ht]
    \centerline{\includegraphics[width=.8\textwidth]{new_tree.png}}
    % \vspace*{-2mm}
    \caption{Extended guidance diagram for picking a good starting configuration given dataset characteristics and a target metric.}
    %% Breakdown of optimal ensembles with respect to metric of choice and dataset configuration.
    %% Edges connecting leaf nodes correspond to Outcome and Volatility metrics described in the previous section.
    %% Each leaf node lists model configurations using the notation
    %% introduced in Fig.~\ref{fig:standard_model}.}
    \label{fig:large-tree}
    % \vspace*{-2mm}
\end{figure*}
